Attacking the Diebold Signature Variant -- RSA Signatures with Unverified High-order Padding

We examine a natural but improper implementation of RSA signature verification deployed on the widely used Diebold Touch Screen and Optical Scan voting machines. In the implemented scheme, the verifier fails to examine a large number of the high-order bits of signature padding and the public exponent is three. We present an very mathematically simple attack that enables an adversary to forge signatures on arbitrary messages in a negligible amount of time.

==> Makefile <==
TEX-FILES = *.tex *.bib
PDF-FILE  = *.pdf

ROOT-FILE = rsa_padding_attack

pdf:	${TEX-FILES} 
	pdflatex ${ROOT-FILE}
	-bibtex  ${ROOT-FILE}
	pdflatex  ${ROOT-FILE}
	pdflatex  ${ROOT-FILE}


clean:
	rm -f *.aux *.bbl *.blg *.log *.dvi *.bak *.out *~ \#*\#  ${ROOT-FILE}.ps  ${ROOT-FILE}.pdf 

view:	pdf
	 ${ROOT-FILE}.pdf

